Optical selection bias and projection effects in stacked galaxy cluster weak lensing

Cosmological constraints from current and upcoming galaxy cluster surveys are limited by the accuracy of cluster mass calibration. In particular, optically identified galaxy clusters are prone to selection effects that can bias the weak lensing mass calibration. We investigate the selection bias of the stacked cluster lensing signal associated with optically selected clusters, using clusters identified by the redMaPPer algorithm in the Buzzard simulations as a case study. We find that at a given cluster halo mass, the residuals of redMaPPer richness and weak lensing signal are positively correlated. As a result, for a given richness selection, the stacked lensing signal is biased high compared with what we would expect from the underlying halo mass probability distribution. The cluster lensing selection bias can thus lead to overestimated mean cluster mass and biased cosmology results. We show that the lensing selection bias exhibits a strong scale-dependence and is approximately 20 to 60 percent for $\Delta\Sigma$ at large scales. This selection bias largely originates from spurious member galaxies within +/- 20 to 60 Mpc/h along the line of sight, highlighting the importance of quantifying projection effects associated with the broad redshift distribution of member galaxies in photometric cluster surveys. While our results qualitatively agree with those in the literature, accurate quantitative modelling of the selection bias is needed to achieve the goals of cluster lensing cosmology and will require synthetic catalogues covering a wide range of galaxy-halo connection models.

==> optical cluster selection bias arxiv v2/authors.tex <==
\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
Hao-Yi~Wu,$^{1}$\thanks{Email: hywu@boisestate.edu}
Matteo~Costanzi,$^{2,3,4}$
Chun-Hao~To,$^{5,6,7}$
Andr\'{e}s~N.~Salcedo,$^{8}$
David~H.~Weinberg,$^{5,6,7}$ \\
James~Annis,$^{9}$
Sebastian~Bocquet,$^{10}$
Maria~Elidaiana~da~Silva~Pereira,$^{11}$
Joseph~DeRose,$^{12}$
Johnny~Esteves,$^{13}$ \\
Arya~Farahi,$^{14}$
Sebastian~Grandis,$^{10}$
Eduardo~Rozo,$^{8}$
Eli~S.~Rykoff,$^{15,16}$
Tam\'{a}s~N.~Varga,$^{17,18}$ \\
Risa~H.~Wechsler,$^{15,16,19}$
Chenxiao~Zeng,$^{5,6}$
Yuanyuan~Zhang,$^{9}$
and Zhuowen~Zhang$^{20}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ Department of Physics, Boise State University, Boise, ID 83725, USA\\
$^{2}$ Astronomy Unit, Department of Physics, University of Trieste, via Tiepolo 11, I-34131 Trieste, Italy\\
$^{3}$ INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{4}$ Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{5}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{6}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{7}$ Department of Astronomy, The Ohio State University, Columbus, OH 43210, USA\\
$^{8}$ Department of Physics, University of Arizona, Tucson, AZ 85721, USA\\
$^{9}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{10}$ University Observatory, Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{11}$ Hamburger Sternwarte, Universit\"{a}t Hamburg, Gojenbergsweg 112, 21029 Hamburg, Germany\\
$^{12}$ Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA\\
$^{13}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{14}$ Departments of Statistics and Data Science, University of Texas at Austin, Austin, TX 78757, USA\\
$^{15}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{16}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{17}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{18}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
$^{19}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{20}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
}
}

==> optical cluster selection bias arxiv v2/mycommand_selection.tex <==


\newcommand{\avg}[1]{\left\langle{#1}\right\rangle}
%\newcommand{\comment}[1]{}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{equation}\begin{aligned}}
\newcommand{\eeqa}{\end{aligned}\end{equation}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}

\newcommand{\hiGpc}{h^{-1} \rm Gpc}
\newcommand{\hiMpc}{h^{-1} \rm Mpc}
\newcommand{\hikpc}{h^{-1} \rm kpc}
\newcommand{\hiMsun}{h^{-1} M_\odot}
\newcommand{\Msun}{M_\odot}

% for cov paper
\newcommand{\Cov}{{\rm Cov}}
\newcommand{\DS}{\Delta\Sigma}
\newcommand{\Sigcrit}{\Sigma_{\rm crit}}

\newcommand{\clhh}{C_\ell^{\rm hh}}
\newcommand{\clkk}{C_\ell^{\kappa\kappa}}
\newcommand{\clhk}{C_\ell^{\rm h\kappa}}

\newcommand{\clSS}{C_\ell^{\Sigma\Sigma}}
\newcommand{\clhS}{C_\ell^{\rm h\Sigma}}

\newcommand{\fsky}{f_{\rm sky}}
\newcommand{\nside}{n_{\rm side}}
\newcommand{\psrc}{p_{\rm src}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\thetamin}{\theta_{\rm min}}
\newcommand{\thetamax}{\theta_{\rm max}}





\newcommand{\tu}{\tilde{u}}

\newcommand{\rp}{r_{\rm p}}


\newcommand{\Pmm}{P_{\rm mm}}
\newcommand{\Phm}{P_{\rm hm}}


%% raised chi (making subscript prettier)
\DeclareRobustCommand{\rchi}{{\mathpalette\irchi\relax}}
\newcommand{\irchi}[2]{\raisebox{\depth}{$#1\chi$}} 

\newcommand{\chis}{\rchi_{\rm s}}
\newcommand{\chih}{\rchi_{\rm h}}
\newcommand{\chiLSS}{\rchi_{\rm lss}}

\newcommand{\chimin}{\rchi_{\rm min}}
\newcommand{\chimax}{\rchi_{\rm max}}

\newcommand{\zs}{z_{\rm s}}
\newcommand{\zh}{z_{\rm h}}
\newcommand{\zLSS}{z_{\rm lss}}

\newcommand{\Ci}{{\rm Ci}}
\newcommand{\Si}{{\rm Si}}



\newcommand{\nh}{n_{\rm h}^{\rm (2D)}}
\newcommand{\ns}{n_{\rm s}^{\rm (2D)}}


\newcommand{\dd}{{\rm d}}
\newcommand{\xihm}{\xi_{\rm hm}}
%\newcommand{\xicm}{\xi_{\rm cm}}

\newcommand{\sigmaf}{\sigma_{f}}






\newcommand{\cvir}{c_\mathrm{vir}}

\newcommand{\chisqc}{\chi^2_{\rm color}}

%\newcommand{\gammat}{\gamma_{\rm t}}

\newcommand{\lnM}{{\rm lnM}}
\newcommand{\lnL}{{\rm ln\lambda}}
\newcommand{\lnS}{{\rm ln\Sigma}}
\newcommand{\lnW}{{\rm ln M_{wl}}}
\newcommand{\dlnL}{{\rm\Delta ln\lambda}}
\newcommand{\dlnS}{{\rm\Delta ln\Sigma}}
\newcommand{\dlnW}{{\rm\Delta lnM_{wl}}}


\newcommand{\sigL}{\sigma_{\rm ln\lambda}}
\newcommand{\sigS}{\sigma_{\rm ln\Sigma}}
\newcommand{\sigW}{\sigma_{\rm ln M_{wl}}}
\newcommand{\Lmin}{\lambda_{\rm min}}
\newcommand{\Lmax}{\lambda_{\rm max}}
\newcommand{\Mwl}{M_{\rm wl}}
\newcommand{\lnMwl}{{\rm ln M_{\rm wl}}}
%%%%


\newcommand{\sigmaz}{\sigma_z}

\newcommand{\Mvir}{M_{\rm vir}}
\newcommand{\Rvir}{R_{\rm vir}}
\newcommand{\cosi}{\cos(i)}
\newcommand{\lammin}{\lambda_{\rm min}}
\newcommand{\lammax}{\lambda_{\rm max}}

\newcommand{\Rlambda}{R_{\lambda}}



\newcommand{\redmapper}{redMaPPer\xspace} % \xspace add space after the command
\newcommand{\redmagic}{redMaGiC\xspace}


